Spotlight and Shadow: Attention-Guided Dual-Anchor Introspective Decoding for MLLM Hallucination Mitigation

Multimodal Large Language Models (MLLMs) have demonstrated remarkable reasoning capabilities yet continue to suffer from hallucination, where generated text contradicts visual content. In this paper, we introduce Dual-Anchor Introspective Decoding (DaID), a novel contrastive decoding framework that dynamically calibrates each token generation by mining the model's internal perceptual discrepancies. Specifically, DaID identifies a Spotlight layer to amplify visual factual signals and a Shadow layer to suppress textual inertia. By leveraging visual attention distributions to guide this dual-anchor selection process, our method ensures precise, token-specific adaptation. Experimental results across multiple benchmarks and MLLMs demonstrate that DaID significantly mitigates hallucination while enhancing general reasoning capabilities.

==> Table/table_layer_merge.tex <==
\begin{table}[!t]
% \small
\centering
\renewcommand{\arraystretch}{0.9}  % 设置行间距为 1.5 倍

\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Method}}  & \multicolumn{4}{c}{\textbf{Close-Ended Benchmark}} &\multirow{2}{*}{\textbf{Average}} \\  

\cmidrule{2-5}

& \textbf{TruthfulQA} & \textbf{MMLU} & \textbf{IFEval} & \textbf{BBH}   \\ 
% \midrule[1pt]
% \multicolumn{6}{c}{\textbf{TinyLLaMA}} \\ 
% \midrule[1pt]

% w/o global           &  &  &  &  &  \\ 
% w/o local            &  &  &  &  &  \\
% \rowcolor{cyan!10}
% \textbf{{FedPruner}} &  &  &  &  &  \\

% \hdashline

% w/o global           &  &  &  &  &  \\ 
% w/o local            &  &  &  &  &  \\
% \rowcolor{cyan!10}
% \textbf{{FedPruner}$^{fine}$} &  &  &  &  &  \\

\midrule[1pt]
&\multicolumn{4}{c}{\textbf{LLaMA2-7B (INT4)}} &\\ 
\midrule[1pt]
\rowcolor{mygreen!10}
{w/o SII} & 48.04 & 43.26 & 31.63 & 39.38 & 40.58 \\
\hdashline
$K=1$ & 48.76 & 43.34 & 32.57 & 39.85 & 41.13 \textcolor{orange}{($\uparrow$ 0.55)} \\ 
$K=2$  & 49.82 & 43.55 & 33.41 & 40.59 & 41.84 \textcolor{orange}{($\uparrow$ 1.26)} \\
% \rowcolor{cyan!5}
$K=3$  & \textbf{50.19} & \textbf{44.18} & \textbf{33.85} & \textbf{40.92} & \textbf{42.29} \textcolor{orange}{($\uparrow$ 1.71)} \\
$K=4$  & 48.33 & 43.07 & 31.92 & 39.16 & 40.62 \textcolor{orange}{($\uparrow$ 0.04)} \\
\midrule[1pt]
&\multicolumn{4}{c}{\textbf{LLaMA2-13B (INT4)}} &\\ 
\midrule[1pt]
\rowcolor{mygreen!10}
w/o SII & 54.46 & 56.34 & 42.68 & 46.65 & 50.03 \\
\hdashline
$K=1$  & 55.18 & 57.02 & 44.15 & 47.48 & 50.96 \textcolor{orange}{($\uparrow$ 0.93)} \\
$K=2$ & 56.01 & 57.99 & 45.48 & 48.39 & 51.97 \textcolor{orange}{($\uparrow$ 1.94)} \\
% \rowcolor{cyan!5}
$K=3$ & \textbf{57.23} & \textbf{58.77} & \textbf{46.51} & \textbf{48.82} & \textbf{52.83} \textcolor{orange}{($\uparrow$ 2.80)} \\
$K=4$ & 54.84 & 56.68 & 43.37 & 46.55 & 50.36 \textcolor{orange}{($\uparrow$ 0.33)} \\
\bottomrule[1pt]
\end{tabular}
}
\vspace{-2mm}
\caption{Effectiveness of the semantic information integration strategy and the impact of varying $K$ values.}
\label{Tab:layer_merge}
\vspace{-6mm}
\end{table}

==> Table/table_main2.tex <==
\definecolor{steelbluev2}{HTML}{DAE8FC}
\definecolor{steelblue}{HTML}{82B0D2}
\definecolor{color3}{HTML}{FEFAE0}
\newcolumntype{a}{>{\columncolor{green!10}}c}
\newcolumntype{b}{>{\columncolor{blue!10}}c}
\newcolumntype{d}{>{\columncolor{color3}}c}
\begin{table}[t!]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{POPE}} & \multicolumn{2}{c}{\textbf{CHAIR}} \\
 & Acc.$\uparrow$ & F1$\uparrow$ & CHAIR$_S$$\downarrow$ & CHAIR$_I$$\downarrow$ \\
\midrule
\midrule
\multicolumn{5}{c}{LLaVA-1.5-7B} \\
\midrule

Greedy & 81.4 & 82.2 & 49.6 & 14.4 \\
Beam Search & 84.7 & 84.6 & 46.3 & 12.9\\

\hdashline

Dola & 84.1 & 84.6 & 47.1 & 13.8 \\
VCD  & 84.7 & 84.5 & 49.2 & 14.8 \\
HALC & 83.9 & 84.0 & 50.2 & 12.4 \\
OPERA & 84.9 & 85.2 & 45.4 & 12.7 \\
SID & 84.8 & 85.5 & 44.2 & 12.2 \\
RITUAL & 84.3 & 85.2 & 45.2 & 13.2 \\
DOPRA & 84.3 & 84.6 & 46.3 & 13.8 \\

\hdashline

\rowcolor{gray!10} \our & 85.1 & 85.9 & 35.9 & 11.3 \\
\midrule
\midrule
\multicolumn{5}{c}{LLaVA-Next} \\
\midrule
Greedy & 83.8 & 82.2 & 32.8 & 9.1 \\
Beam Search & 83.8 & 81.7 & 33.0 & 9.2 \\

\hdashline

Dola & 84.5 & 84.8 & 31.3 & 9.0 \\
VCD  & 83.4 & 84.0 & 32.8 & 8.9  \\
HALC & \\
OPERA & 84.4 & 84.2 & 34.0 & 8.7 \\
SID & 84.6 & 85.3 & 32.8 & 8.3 \\
RITUAL & \\
DOPRA &  \\

\hdashline

\rowcolor{gray!10} \our & 85.3 & 85.8 & 24.2 & 8.2 \\

\midrule
\midrule
\multicolumn{5}{c}{Qwen-VL} \\
\midrule
Greedy & \\
Beam Search & \\

\hdashline

Dola &  \\
VCD  & \\
HALC & \\
OPERA & \\
SID & \\
RITUAL & \\
DOPRA &  \\

\hdashline

\rowcolor{gray!10} \our & \\
\bottomrule

\end{tabular}%
}
\caption{Compare results of \our with other SOTA methods on POPE, CHAIR and MME benchmarks. The best performances within each setting are \textbf{bolded}, and the model is LLaVA-1.5-7B.}
\label{tab:main_results}
\end{table}

==> Table/table_other_benchmark.tex <==
\begin{table}[t!]
\centering
\caption{Benchmark results on general vision-language task.}
\label{tab:benchmark_results}
% 减小列间距以适应单栏宽度
\setlength{\tabcolsep}{3.5pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Model} & \textbf{GQA}$\uparrow$ & \textbf{VizWiz}$\uparrow$ & \textbf{MMB}$\uparrow$ & \textbf{SEED$^{\text{I}}$}$\uparrow$ \\ 
\midrule
LLaVA-1.5-7B & 62.0 & 50.0 & 64.3 & 58.6 \\
\rowcolor{gray!10} \textbf{+ Ours} \\
\hdashline
LLaVA-1.5-13B & 63.3 & 53.6 & 67.7 & 61.6 \\
\rowcolor{gray!10} \textbf{+ Ours} \\
\hdashline
Qwen2-VL-7B & 64.5 & 65.4 & 83.0 & 77.9 \\
\rowcolor{gray!10} \textbf{+ Ours} \\
\hdashline
InternVL2-8B & 63.2 & 63.0 & 81.7 & 76.2 \\
\rowcolor{gray!10} \textbf{+ Ours} \\ 
\bottomrule
\end{tabular}%
}
\end{table}

==> Table/table_other_benchmark_new.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.5\textwidth}{!}{%
        \begin{tabular}{lcccccccccc}
            \toprule
            \textbf{Model} & \textbf{GQA} & \textbf{VQA$^{\text{v2}}$} & \textbf{MMB} & \textbf{SEED$^{\text{I}}$} & \textbf{VizWiz}\\
            \midrule
            LLaVA-1.5-7B & 62.0 & 78.5 & 64.3 & 58.6 & 50.0\\
            \rowcolor{gray!10} \textbf{+ Ours} & 63.2 & 78.9 & 65.9 & 60.7 & 51.1\\
            \hline
            LLaVA-1.5-13B & 63.3 & 80.0 & 67.7 & 61.6 &  53.6 \\
            \rowcolor{gray!10} \textbf{+ Ours} & 64.6 & 81.3 & 68.9 & 62.4 & 54.3 \\
            \bottomrule
        \end{tabular}%
    }
    \caption{Benchmark results on general vision-language task.}
    \label{tab:benchmark_results}
\end{table}

==> Table/table_other_models.tex <==
\definecolor{impblue}{HTML}{0000FF}
\definecolor{new_color}{HTML}{e7e7de}

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccc}
\toprule
% --- 修改了下面这一行 ---
Model & CHAIR$_S$$\downarrow$ & CHAIR$_I$$\downarrow$ & POPE-F1$\uparrow$ \\ 
\midrule
Qwen2-VL & 25.0 & 7.3 & 86.6 \\
\rowcolor{new_color} + \textbf{\our} & \textbf{23.6} \textcolor{impblue}{(-1.4)} & \textbf{6.3} \textcolor{impblue}{(-1.0)} & \textbf{87.5} \textcolor{impblue}{(+0.9)} \\
% QwenVL-Chat & 45.6 & 12.5 & 87.0 \\
% \rowcolor{new_color} + \textbf{\our} & \textbf{} \textcolor{impblue}{(+)} & \textbf{} \textcolor{impblue}{(+)} & \textbf{} \textcolor{impblue}{(+)} \\
MiniGPT-4 & 31.8 & 9.9 & 70.3 \\
\rowcolor{new_color} + \textbf{\our} & \textbf{29.9} \textcolor{impblue}{(-1.9)} & \textbf{8.1} \textcolor{impblue}{(-1.8)} & \textbf{71.1} \textcolor{impblue}{(+0.8)} \\
InstructBLIP & 58.8 & 23.7 & 84.4 \\
\rowcolor{new_color} + \textbf{\our} & \textbf{55.2} \textcolor{impblue}{(-3.6)} & \textbf{18.4} \textcolor{impblue}{(-5.3)} & \textbf{86.3} \textcolor{impblue}{(+1.9)} \\
% Shikra & 55.8 & 15.4 & 82.5 \\
% \rowcolor{new_color} + \textbf{\our} & \textbf{} \textcolor{impblue}{(+)} & \textbf{} \textcolor{impblue}{(+)} & \textbf{} \textcolor{impblue}{(+)} \\
Mini-Gemini & 32.6 & 8.7 & 85.6 \\
\rowcolor{new_color} + \textbf{\our} & \textbf{} \textcolor{impblue}{(+)} & \textbf{} \textcolor{impblue}{(+)} & \textbf{} \textcolor{impblue}{(+)} \\
% LLaVA1.5 & 47.0 & 13.8 & 84.9 \\
% \rowcolor{new_color} + \textbf{\our} & \textbf{} \textcolor{impblue}{(+)} & \textbf{} \textcolor{impblue}{(+)} & \textbf{} \textcolor{impblue}{(+)} \\
% LLaVA1.6 & 42.6 & 14.4 & 86.5 \\
% \rowcolor{new_color} + \textbf{\our} & \textbf{} \textcolor{impblue}{(+)} & \textbf{} \textcolor{impblue}{(+)} & \textbf{} \textcolor{impblue}{(+)} \\
InternVL & 45.8 & 12.9 & 86.4 \\
\rowcolor{new_color} + \textbf{\our} & \textbf{} \textcolor{impblue}{(+)} & \textbf{} \textcolor{impblue}{(+)} & \textbf{} \textcolor{impblue}{(+)} \\
\bottomrule
\end{tabular}
}
\caption{Generalization analysis of \our across diverse MLLM architectures on CHAIR and POPE benchmarks.}
\label{tab:generalization_study}
\end{table}

==> Table/table_sensitivity_alpha.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{0.85} 
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{$\alpha$}} & \multicolumn{2}{c}{LLaVA-1.5} &  \multicolumn{2}{c}{LLaVA-NeXT} \\
& POPE-F1$\uparrow$ & POPE-Acc.$\uparrow$ & POPE-F1$\uparrow$ & POPE-Acc.$\uparrow$\\
\midrule
0.4 & 83.63 & 83.44 & 84.06 & 84.24 \\
0.6 & 84.14 & 83.98 & 85.00 & 84.93 \\
0.8 & 85.92 & 85.08 & 85.76 & 85.32 \\
1.0 & 85.21 & 84.59 & 84.10 & 84.25 \\
1.2 & 84.20 & 83.72 & 84.09 & 83.78\\
\bottomrule
\end{tabular}%
}
\caption{Sensitivity analysis of visual perception reinforcement intensity $\alpha$ on LLaVA-1.5 and LLaVA-NeXT.}
\label{tab:sensitivity_alpha}
\end{table}

==> Table/table_sensitivity_beta.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{0.85} 
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{$\beta$}} & \multicolumn{2}{c}{LLaVA-1.5} &  \multicolumn{2}{c}{LLaVA-NeXT} \\
& POPE-F1$\uparrow$ & POPE-Acc.$\uparrow$ & POPE-F1$\uparrow$ & POPE-Acc.$\uparrow$\\
\midrule
0.0 & 84.99 & 84.57 & 85.29 & 84.93\\
0.2 & 85.92 & 85.08 & 85.76 & 85.32 \\
0.4 & 84.03 & 83.89 & 84.25 & 83.88 \\
0.6 & 82.17 & 82.01 & 82.37 & 82.12\\

\bottomrule
\end{tabular}%
}
\caption{Sensitivity analysis of the language prior suppression intensity $\beta$ on LLaVA-1.5 and LLaVA-NeXT.}
\label{tab:sensitivity_beta}
\end{table}

==> Table/table_submodel_construction.tex <==
\begin{table}[!t]
\small
\renewcommand{\arraystretch}{1.0}  % 设置行间距为 1.5 倍
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Method}}  & \multicolumn{4}{c}{\textbf{Close-Ended Benchmark}} &\multirow{2}{*}{\textbf{Average}} \\  

\cmidrule{2-5}

& \textbf{TruthfulQA} & \textbf{MMLU} & \textbf{IFEval} & \textbf{BBH}   \\ 
% \midrule[1pt]
% \multicolumn{6}{c}{\textbf{TinyLLaMA}} \\ 
% \midrule[1pt]

% w/o global           &  &  &  &  &  \\ 
% w/o local            &  &  &  &  &  \\
% \rowcolor{cyan!10}
% \textbf{{FedPruner}} &  &  &  &  &  \\

% \hdashline

% w/o global           &  &  &  &  &  \\ 
% w/o local            &  &  &  &  &  \\
% \rowcolor{cyan!10}
% \textbf{{FedPruner}$^{fine}$} &  &  &  &  &  \\

\midrule[1pt]
&\multicolumn{4}{c}{\textbf{LLaMA2-7B (INT4)}} &\\ 
\midrule[1pt]
\rowcolor{mygreen!10}
w/o TLP        & 45.37 & 41.97 & 30.17 & 38.72 & 39.06 \\
\hdashline
$\beta=90\%$         & 46.54 & 42.73 & 31.25 & 39.35 & 39.97 \textcolor{orange}{($\uparrow$ 0.91)} \\ 
$\beta=80\%$         & 48.26 & 43.65 & 32.46 & 40.15 & 41.13 \textcolor{orange}{($\uparrow$ 2.07)} \\
$\beta=70\%$         & \textbf{50.19} & \textbf{44.18} & \textbf{33.85} & \textbf{40.92} & \textbf{42.29} \textcolor{orange}{($\uparrow$ 3.23)} \\
$\beta=60\%$         & 47.95 & 43.27 & 32.14 & 39.86 & 40.81 \textcolor{orange}{($\uparrow$ 1.75)}\\
$\beta=50\%$         & 46.08 & 42.51 & 31.08 & 39.22 & 39.72 \textcolor{orange}{($\uparrow$ 0.66)} \\

\midrule[1pt]
&\multicolumn{4}{c}{\textbf{LLaMA2-13B (INT4)}} &\\ 
\midrule[1pt]
\rowcolor{mygreen!10}
w/o TLP        & 51.92 & 54.05 & 41.26 & 45.53 & 48.19 \\
\hdashline
$\beta=90\%$        & 53.47 & 55.48 & 42.83 & 46.42 & 49.55 \textcolor{orange}{($\uparrow$ 1.36)} \\ 
$\beta=80\%$         & 54.89 & 56.82 & 44.29 & 47.11 & 50.78 \textcolor{orange}{($\uparrow$ 2.59)} \\
$\beta=70\%$         & 56.12 & 57.96 & 45.48 & 48.07 & 51.91 \textcolor{orange}{($\uparrow$ 3.72)} \\
$\beta=60\%$         & \textbf{57.23} & \textbf{58.77} & \textbf{46.51} & \textbf{48.82} & \textbf{52.83} \textcolor{orange}{($\uparrow$ 4.64)} \\
$\beta=50\%$         & 55.83 & 57.26 & 45.18 & 47.93 & 51.55 \textcolor{orange}{($\uparrow$ 3.36)}\\
\bottomrule[1pt]
\end{tabular}
}
\vspace{-2mm}
\caption{Effectiveness of the task-oriented layer prioritization mechanism and the impact of varying $\beta$ values.}
\label{submodel_construction}
\vspace{-2mm}
\end{table}

==> graph/Figure_motivation.tex <==
% 定义颜色
\definecolor{llava15}{RGB}{46,134,171}  % #2E86AB
\definecolor{llavanext}{RGB}{242,66,54}  % #F24236

\begin{figure}[!t]
\centering
\begin{tikzpicture}
    % 第一个子图：Hallucination Rate
    \begin{axis}
    [
        anchor=north west,
        at={(0em,0em)},
        ymajorgrids,
        xmajorgrids,
        grid style={dashed, gray!40},
        width=0.48\columnwidth,
        height=0.25\columnwidth,
        xmin=0,
        xmax=34,
        ymin=0,
        ymax=65,
        xtick={0,4,8,12,16,20,24,28,32},
        ytick={0,10,20,30,40,50,60},
        xlabel={Layer Index},
        xlabel style={font=\small\bfseries, yshift=0.3em},
        ylabel={Hallucination Rate (\%)},
        ylabel style={font=\small\bfseries, xshift=-0.3em},
        legend style={
            at={(0.98,0.98)},
            anchor=north east,
            font=\small,
            cells={anchor=west},
            fill opacity=0.95,
            draw=gray,
            fill=white
        },
        axis line style={line width=1.2pt},
        tick style={line width=1.2pt},
        ticklabel style={font=\small},
        every axis plot/.append style={line width=2.5pt}
    ]

        % LLaVA-1.5: 方形标记，深蓝色
        \addplot[
            llava15,
            mark=square*,
            mark size=2.5pt,
            mark options={fill=llava15, draw=white, line width=1pt},
            thick
        ] coordinates {
            (1, 56.52) (2, 60.87) (3, 56.52) (4, 56.52) (5, 60.87) (6, 52.17) (7, 39.13) (8, 43.48) (9, 34.78) (10, 26.09) (11, 21.74) (12, 21.74) (13, 21.74) (14, 21.74) (15, 17.39) (16, 17.39) (17, 21.74) (18, 21.74) (19, 21.74) (20, 21.74) (21, 17.39) (22, 17.39) (23, 17.39) (24, 17.39) (25, 13.04) (26, 13.04) (27, 13.04) (28, 13.04) (29, 17.39) (30, 13.04) (31, 17.39) (32, 21.74)
        };
        \addlegendentry{LLaVA-1.5}

        % LLaVA-NeXT: 圆形标记，红色
        \addplot[
            llavanext,
            mark=*,
            mark size=2.5pt,
            mark options={fill=llavanext, draw=white, line width=1pt},
            thick
        ] coordinates {
            (1, 38.89) (2, 44.44) (3, 44.44) (4, 44.44) (5, 44.44) (6, 44.44) (7, 27.78) (8, 38.89) (9, 33.33) (10, 33.33) (11, 33.33) (12, 27.78) (13, 27.78) (14, 27.78) (15, 27.78) (16, 27.78) (17, 27.78) (18, 27.78) (19, 27.78) (20, 27.78) (21, 33.33) (22, 38.89) (23, 38.89) (24, 38.89) (25, 38.89) (26, 38.89) (27, 38.89) (28, 38.89) (29, 38.89) (30, 38.89)
        };
        \addlegendentry{LLaVA-NeXT}

    \end{axis}

    % 第二个子图：Accuracy（垂直排列在第一个图下方）
    \begin{axis}
    [
        anchor=north west,
        at={(0em,-6.5em)},
        ymajorgrids,
        xmajorgrids,
        grid style={dashed, gray!40},
        width=0.48\columnwidth,
        height=0.25\columnwidth,
        xmin=0,
        xmax=34,
        ymin=55,
        ymax=90,
        xtick={0,4,8,12,16,20,24,28,32},
        ytick={55,60,65,70,75,80,85,90},
        xlabel={Layer Index},
        xlabel style={font=\small\bfseries, yshift=0.3em},
        ylabel={Accuracy (\%)},
        ylabel style={font=\small\bfseries, xshift=-0.3em},
        legend style={
            at={(0.98,0.02)},
            anchor=south east,
            font=\small,
            cells={anchor=west},
            fill opacity=0.95,
            draw=gray,
            fill=white
        },
        axis line style={line width=1.2pt},
        tick style={line width=1.2pt},
        ticklabel style={font=\small},
        every axis plot/.append style={line width=2.5pt}
    ]

        % LLaVA-1.5: 方形标记，深蓝色
        \addplot[
            llava15,
            mark=square*,
            mark size=2.5pt,
            mark options={fill=llava15, draw=white, line width=1pt},
            thick
        ] coordinates {
            (1, 60.00) (2, 60.00) (3, 64.44) (4, 64.44) (5, 62.22) (6, 66.67) (7, 73.33) (8, 71.11) (9, 75.56) (10, 82.22) (11, 84.44) (12, 84.44) (13, 84.44) (14, 82.22) (15, 84.44) (16, 86.67) (17, 84.44) (18, 84.44) (19, 82.22) (20, 82.22) (21, 84.44) (22, 84.44) (23, 84.44) (24, 84.44) (25, 86.67) (26, 86.67) (27, 86.67) (28, 86.67) (29, 84.44) (30, 86.67) (31, 84.44) (32, 82.22)
        };
        \addlegendentry{LLaVA-1.5}

        % LLaVA-NeXT: 圆形标记，红色
        \addplot[
            llavanext,
            mark=*,
            mark size=2.5pt,
            mark options={fill=llavanext, draw=white, line width=1pt},
            thick
        ] coordinates {
            (1, 72.22) (2, 69.44) (3, 63.89) (4, 66.67) (5, 69.44) (6, 69.44) (7, 77.78) (8, 69.44) (9, 72.22) (10, 72.22) (11, 75.00) (12, 77.78) (13, 77.78) (14, 75.00) (15, 77.78) (16, 77.78) (17, 80.56) (18, 80.56) (19, 80.56) (20, 80.56) (21, 75.00) (22, 72.22) (23, 72.22) (24, 72.22) (25, 69.44) (26, 69.44) (27, 69.44) (28, 69.44) (29, 66.67) (30, 69.44)
        };
        \addlegendentry{LLaVA-NeXT}

    \end{axis}
\end{tikzpicture}
\vspace{-2mm}
\caption{Layer-wise analysis of MLLM behavior. (Top) Hallucination rate decreases monotonically with layer depth, with shallow layers exhibiting the most severe hallucination tendencies. (Bottom) Object recognition accuracy follows an inverted-U trajectory, peaking in middle-to-deep layers before declining in final layers due to textual inertia.}
\label{fig:motivation}
\vspace{-4mm}
\end{figure}


==> section/Experiments_old.tex <==
\section{Experiments}

\subsection{Experimental Settings}

\paragraph{Baselines.}
We compare \our with the following baselines.
1) DoLa~\cite{chuang2023dola} contrasts early and late layers to isolate factual knowledge; 
2) VCD~\cite{leng2024mitigating} mitigates hallucination by contrasting original and distorted visual inputs; 
3) OPERA~\cite{huang2024opera} employs an attention penalty to prevent token over-trust; 
4) SID~\cite{huo2024self} exploits internal state discrepancies for intrinsic correction; 
% 5) DeCo~\cite{wang2024mllm} rectifies outputs by anchoring to a heuristically selected layer; 
and 5) EAZY~\cite{che2025hallucinatory} eliminates hallucinations by zeroing out hallucinatory image tokens.


\paragraph{Evaluation Models.} We validate \our across five representative MLLMs: LLaVA-1.5~\cite{liu2023visual}, LLaVA-NeXT~\cite{li2024llavanext-strong}, Qwen2-VL~\cite{wang2024qwen2}, MiniGPT-4~\cite{zhu2023minigpt}, and InstructBLIP~\cite{dai2023instructblip}. All models are evaluated at the 7B parameter scale.


\paragraph{Implementation Details.} All experiments are implemented using the PyTorch and Hugging Face Transformers libraries. We conduct evaluations on NVIDIA RTX 5070 Ti GPUs. For the dual-anchor contrastive decoding, we set $\alpha = 0.8$ to govern the intensity of visual perception reinforcement and $\beta = 0.2$ to modulate the suppression of linguistic priors. Additionally, the confidence threshold for the adaptive plausibility constraint is set to $\gamma = 0.9$ for the POPE benchmark and 0.1 for others, ensuring that the dual-anchor adjustments are confined to a linguistically valid candidate set.

% we configure the hyperparameters to balance visual perception fidelity and linguistic coherence. Specifically, 

\subsection{Benchmarks and Metrics}
\label{sec:benchmarks}

To conduct a comprehensive evaluation, we utilize three visual hallucination benchmarks alongside five general vision-language benchmarks.

% To conduct a comprehensive evaluation, we employ eight mainstream multimodal benchmarks, including three visual hallucination tasks and five general vision-language tasks. 

\paragraph{Visual Hallucination Tasks.} These benchmarks evaluate the consistency between model responses and image content.
\begin{itemize}
    \item \textbf{POPE}~\cite{li2023evaluating}: Assesses object hallucination by asking binary questions (e.g., \texttt{"Is there a <object> in the image?"}). We report the Accuracy and F1 score.
    \item \textbf{CHAIR}~\cite{rohrbach2018object}: Evaluates object hallucination in image captioning by comparing generated descriptions against ground-truth annotations. We report the $\text{CHAIR}_I$ (Eq.~\eqref{eq:chair1}) and $\text{CHAIR}_S$ (Eq.~\eqref{eq:chair2}).
    \item \textbf{MME}~\cite{fu2025mme}: Measures perceptual and cognitive abilities. We focus on the object-level (Existence, Count) and attribute-level (Position, Color) subsets, reporting the corresponding perception score.
\end{itemize}
\begin{equation}
    \text{CHAIR}_{\text{I}} = \frac{|\{\text{hallucinated objects}\}|}{\text{all mentioned objects}}.
\label{eq:chair1}
\end{equation}
\begin{equation}
    \text{CHAIR}_{\text{S}}= \frac{|\{\text{captions with hallucinated objects}\}|}{\text{all captions}}.
\label{eq:chair2}
\end{equation}

\paragraph{General Vision-Language Tasks.} To assess the comprehensive multimodal reasoning capabilities of MLLMs, we evaluate accuracy across five widely adopted benchmarks
% To assess the comprehensive multimodal reasoning of MLLMs, we evaluate the Accuracy across five widely adopted benchmarks.
\begin{itemize}
    \item \textbf{GQA}~\cite{hudson2019gqa}: Focuses on visual reasoning and compositional question answering through image scene graphs.
    \item \textbf{VQA$^{\text{v2}}$}~\cite{goyal2017making}: A standard benchmark requiring open-ended visual question answering grounded in image content.
    \item \textbf{MMB}~\cite{liu2024mmbench}: Evaluates 20 ability dimensions using a circular strategy.
    \item \textbf{Seed$^I$}~\cite{li2023seed}: Assesses  generative comprehension and spatial relationship understanding via multiple-choice questions.
    \item \textbf{VizWiz}~\cite{gurari2018vizwiz}: Tests the model's ability to resolve diverse visual queries originating from blind individuals.
\end{itemize}



% \begin{itemize}
%     \item \textbf{GQA}~\cite{hudson2019gqa}: A dataset for real-world visual reasoning and compositional question answering based on image scene graphs, evaluated using Accuracy.
%     \item \textbf{VQA$^{\text{v2}}$}~\cite{goyal2017making}: A standard visual question answering benchmark that requires models to understand image content to answer open-ended questions, measured by Accuracy.
%     \item \textbf{MMB}~\cite{liu2024mmbench}: MM-Bench assesses 20 different ability dimensions using a circular evaluation strategy and GPT-4 based answer matching to determine Accuracy.
%     \item \textbf{Seed$^I$}~\cite{li2023seed}: SEED-Bench-image evaluates generative comprehension through multiple-choice questions, focusing on the model's spatial relationship and image understanding Accuracy.
%     \item \textbf{VizWiz}~\cite{gurari2018vizwiz}: A benchmark originating from blind people's requests that tests a model's ability to answer visual questions in diverse, real-world scenarios, measured by Accuracy.
% \end{itemize}



% GQA~\cite{hudson2019gqa}, VQA$^{\text{v2}}$~\cite{goyal2017making}, MMB~\cite{liu2024mmbench}, Seed$^{I}$~\cite{li2023seed}, and VizWiz~\cite{gurari2018vizwiz}.




\input{ACL/Table/table_main1}
% \input{ACL/Table/table_other_benchmark_new}
% \input{ACL/Table/table_other_models}

\input{ACL/graph/Figure_other_benchmark}


\subsection{Experimental Results}

\paragraph{Visual Hallucination Tasks.} 
Table~\ref{tab:main_results} provides a comprehensive comparison between \our and existing methods on LLaVA-1.5 and LLaVA-NeXT. \our consistently achieves superior performance across all settings. For instance, on the POPE benchmark for LLaVA-1.5, \our attains a peak accuracy of 85.08\% and an F1-score of 85.92\%, delivering improvements of up to 3.7\% and 3.72\% over baselines, respectively. Notably, \our significantly reduces object hallucinations on the CHAIR benchmark, achieving the lowest $\text{CHAIR}_S$ (35.9\%) and $\text{CHAIR}_I$ (11.3\%). Moreover, \our delivers optimal performance on the MME benchmark. Similar performance gains are also observed on LLaVA-NeXT. These results underscore \our’s exceptional capability in mitigating multimodal hallucinations by reinforcing factual visual grounding while suppressing linguistic priors.


\paragraph{General Vision-Language Tasks.} To ensure that hallucination mitigation does not compromise core reasoning proficiency, we evaluate \our across five general vision-language benchmarks. As illustrated in Figure~\ref{fig:other_bench}, \our not only preserves but consistently enhances general performance across both 7B and 13B scales of LLaVA-1.5. For instance, on Seed$^{I}$, \our achieves a notable margin of +2.1\% at the 7B scale. These results suggest that by amplifying authentic visual signals and filtering out linguistic noise, \our refines the model's internal representational quality. Consequently, our method transcends mere error correction to facilitate a more robust multimodal understanding.

\subsection{Sensitivity Analysis}

In this section, we conduct a sensitivity analysis of \our to the visual reinforcement intensity $\alpha$ and the language prior suppression intensity $\beta$.

\input{ACL/graph/Figure_alpha}
\input{ACL/graph/Figure_beta}
\input{ACL/graph/Figure_other_MLLM}

\paragraph{Visual Perception Reinforcement ($\alpha$).} As shown in Figure~\ref{fig:sensitivity_alpha}, the performance exhibits a distinct bell-shaped trajectory across both models, peaking at $\alpha=0.8$. The initial upward trend confirms that injecting logits from the Spotlight layer effectively counteracts the "seeing-then-forgetting" phenomenon by reintroducing lost visual signals. However, performance degrades when $\alpha$ exceeds 0.8. This decline occurs because the Spotlight layer, while visually rich, is linguistically raw compared to the final layer. An excessively high $\alpha$ causes the unrefined intermediate logits to overpower the final layer's linguistic modeling, disrupting the syntactic coherence of the generated text. Thus, $\alpha=0.8$ represents the optimal equilibrium between visual fidelity and linguistic fluency.


% As shown in Figure~\ref{fig:sensitivity_alpha}, we evaluate the performance of LLaVA-1.5 and LLaVA-Next across various values of $\alpha$. We observe that increasing $\alpha$ generally improves factual consistency (POPE-F1 and Accuracy) as it strengthens the injection of peak visual signals from the intermediate Spotlight layer. However, excessively high values may introduce a slight degradation in performance if the intermediate layer's logits begin to overshadow the final layer's linguistic coherence. The optimal balance is achieved at $\alpha=0.8$.

\paragraph{Language Prior Suppression ($\beta$).} 
Figure~\ref{fig:sensitivity_beta} reveals that the model achieves an optimal peak at $\beta=0.2$. This indicates that a mild penalty is sufficient to neutralize the visual agnosia inherent in the Shadow layer without harming valid generation. Notably, the curve drops sharply as $\beta$ increases beyond 0.2. This sharp decline suggests that aggressive subtraction risks over-penalizing the vocabulary space—stripping away not just the hallucinations driven by textual inertia, but also valid linguistic connectors. Therefore, a low $\beta$ is crucial to surgically excise hallucination noise while preserving the integrity of the decoding distribution.


\subsection{Applicability to Diverse MLLMs}


We further demonstrate the model generalization of \our on a wide spectrum of MLLM architectures, including Qwen2-VL, MiniGPT-4, and InstructBLIP. As illustrated in Figure~\ref{fig:generalization_study}, \our yields consistent and significant performance gains across all evaluated models and benchmarks. Specifically, \our markedly suppresses erroneous object generation. For instance, it achieves a substantial reduction in $\text{CHAIR}_S$ for InstructBLIP (-3.6) and MiniGPT-4 (-1.9), as shown in Figure~\ref{fig:generalization_study}(a). Similarly, a notable drop in $\text{CHAIR}_I$ is observed for InstructBLIP (-5.3) in Figure~\ref{fig:generalization_study}(b). Beyond error reduction, \our consistently bolsters the model's grounding capabilities. On the POPE, we observe significant F1-score improvements, such as +1.9 for InstructBLIP and +0.9 for Qwen2-VL, as depicted in Figure~\ref{fig:generalization_study}(c). 
These results confirm that our attention-guided dual-anchor mechanism serves as a universal, training-free solution for enhancing MLLM reliability.


\subsection{Ablation Study}


\input{ACL/Table/table_ablation}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=1\linewidth]{ACL/graph/Case_study.pdf}
%     \caption{Qualitative case study of \our on a representative instance (input image and query detailed in Figure~\ref{fig_framework}).}
%   \label{fig_case_study}
%   \vspace{-4mm}
% \end{figure*}


\begin{figure*}[!t]
    \centering
    \begin{subfigure}{0.499\textwidth}
        \centering
        \includegraphics[width=\linewidth]{ACL/graph/case_study_main.png}
        \caption{Token probability distribution across layers.}
    \end{subfigure}\hfill
    \begin{subfigure}{0.499\textwidth}
        \centering
        \includegraphics[width=\linewidth]{ACL/graph/case_study_bars.png}
        \caption{Token probabilities for specific layers.}
    \end{subfigure}
    \caption{Qualitative case study of \our on a representative instance (input image and query detailed in Figure~\ref{fig_framework}).}
  \label{fig_case_study}
  \vspace{-3mm}
\end{figure*}

To verify the individual contributions of the dual-anchor components in \our, we conduct ablation experiments on LLaVA-1.5 and LLaVA-NeXT. As summarized in Table~\ref{tab:ablation_results}, removing either the Positive Anchor (PA) or the Negative Anchor (NA) leads to a consistent performance degradation. Specifically, excluding the PA (w/o PA) results in a noticeable decline in POPE accuracy (e.g., from 85.08\% to 83.42\% on LLaVA-1.5). This confirms that reinforcing visual perceptual signals is essential to counteract the "seeing-then-forgetting" phenomenon. Additionally, the absence of the NA (w/o NA) causes a more severe spike in hallucination rates, with $\text{CHAIR}_S$ on LLaVA-1.5 jumping significantly from 35.9 to 47.6. This underscores the necessity of the Shadow layer in isolating and penalizing the linguistic priors. Moreover, \our consistently achieves the best results, significantly outperforming single-anchor variants. This synergy demonstrates that simultaneously amplifying factual visual signals and suppressing linguistic noise is imperative for effective hallucination mitigation.

% To verify the individual contributions of the dual-anchor components in \our, we conduct an ablation study on LLaVA-1.5 and LLaVA-NeXT. The results are summarized in Table~\ref{tab:ablation_results}, comparing \our against variants without the Positive Anchor (PA) or the Negative Anchor (NA). Removing the PA (w/o PA) leads to a noticeable decline in both POPE accuracy and CHAIR scores. This confirms that reinforcing peak perceptual signals from intermediate layers is crucial for preserving authentic visual details that are often "forgotten" in the final layers. The absence of the NA (w/o NA) results in a significant increase in hallucination rates. This demonstrates the necessity of the Shadow layer in isolating and penalizing the unimodal language priors that dominate shallow layers. The full \our configuration consistently outperforms both the "w/o PA" and "w/o NA" variants. This synergy proves that simultaneously amplifying factual signals and suppressing linguistic noise is more effective for hallucination mitigation than relying on a single anchor.


\subsection{Case Study}


Finally, to qualitatively elucidate the mechanistic efficacy of \our, we analyze a representative hallucination instance where the model erroneously prioritizes "reading book" over the visually grounded "using laptop". As shown in Figure~\ref{fig_case_study}(a), the correct token ("using laptop") reaches its probability zenith at layer 25 but is subsequently suppressed by the "reading book" token at the final layer. This visualizes the perceptual-cognitive paradox, where deeper layers prioritize linguistic fluency over intermediate visual evidence. \our adaptively designates layer 2 as the Shadow anchor to capture pure linguistic noise and layer 25 as the Spotlight anchor to amplify visual perceptual signals. Figure~\ref{fig_case_study}(b) shows that \our successfully inverts the erroneous distribution, boosting the correct token's probability from 15.4\% to 39.6\% while effectively suppressing the hallucinated candidate.



